Tripartite Form Universality in Holographic Entropy Inequalities

To elucidate the meaning of holographic entropy inequalities (beyond subadditivity) which characterize the entanglement structure of geometric states in holography, arXiv:2309.06296 proposed the "tripartite form" for these inequalities, consisting of tripartite information and conditional tripartite information terms with unit coefficients. While this provides a compact and useful packaging of the inequalities, it is not a priori guaranteed that all inequalities can be recast in this form. Here we conjecture that they can, and present substantial evidence, by proving that the two known infinite families of holographic entropy inequalities found in arXiv:2309.15145 can indeed be written in the tripartite form. This is significant because such recasting is particularly nontrivial for these families. Apart from providing the explicit tripartite form expressions for every member of these two infinite families, we detail how we arrived at them, in the process deriving several useful identities which may serve as stepping stones to formulate further repackaging of the corresponding information quantities. We also illustrate the power of the tripartite form by proving a number of structural properties satisfied by any holographic entropy inequality.

==> TFmacro.tex <==

% Compact TikZ-backed table helpers for graphical renderin of tripartite form (TF)

\makeatletter
\@ifpackageloaded{fontenc}{}{\RequirePackage[T1]{fontenc}}
\@ifpackageloaded{tikz}{}{\RequirePackage{tikz}}
\@ifpackageloaded{xparse}{}{\RequirePackage{xparse}}
\makeatother

\usetikzlibrary{matrix}

\makeatletter

\newlength{\TFmacroLeftWidth}
\newlength{\TFmacroMiddleWidth}
\newlength{\TFmacroRightWidth}
\newlength{\TFmacroRowHeight}
\newlength{\TFmacroInnerSep}

\setlength{\TFmacroLeftWidth}{0.22\linewidth}
\setlength{\TFmacroMiddleWidth}{0.34\linewidth}
\setlength{\TFmacroRightWidth}{0.26\linewidth}
\setlength{\TFmacroRowHeight}{2.8em}
\setlength{\TFmacroInnerSep}{0.55em}

\definecolor{TFmacroHeaderFill}{RGB}{236,240,244}
\definecolor{TFmacroRule}{RGB}{55,64,72}
\definecolor{TFmacroStripe}{RGB}{248,250,252}

\pgfkeys{
  /TFmacro/.is family,
  /TFmacro,
  left width/.code=\setlength{\TFmacroLeftWidth}{#1},
  middle width/.code=\setlength{\TFmacroMiddleWidth}{#1},
  right width/.code=\setlength{\TFmacroRightWidth}{#1},
  row height/.code=\setlength{\TFmacroRowHeight}{#1},
  inner sep/.code=\setlength{\TFmacroInnerSep}{#1},
  header fill/.code=\colorlet{TFmacroHeaderFill}{#1},
  rule color/.code=\colorlet{TFmacroRule}{#1},
  stripe fill/.code=\colorlet{TFmacroStripe}{#1}
}

\tikzset{
  TFmacro/table/.style={
    matrix of nodes,
    ampersand replacement=\&,
    nodes in empty cells,
    row sep=-\pgflinewidth,
    column sep=-\pgflinewidth,
    nodes={
      draw=TFmacroRule,
      line width=0.45pt,
      minimum height=\TFmacroRowHeight,
      inner xsep=\TFmacroInnerSep,
      inner ysep=0.35em,
      anchor=center,
      text depth=0.25ex,
      text height=1.8ex,
      font=\small,
      align=center
    },
    column 1/.style={nodes={text width=\TFmacroLeftWidth}},
    column 2/.style={nodes={text width=\TFmacroMiddleWidth}},
    column 3/.style={nodes={text width=\TFmacroRightWidth}},
    row 1/.style={nodes={TFmacro/header}}
  },
  TFmacro/header/.style={
    fill=TFmacroHeaderFill,
    font=\small\bfseries,
    line width=0.65pt
  },
  TFmacro/stripe/.style={
    fill=TFmacroStripe
  },
  TFmacro/blank/.style={
    draw=none,
    fill=none,
    minimum height=0.45em,
    inner sep=0pt
  }
}

\NewDocumentCommand{\TFTable}{O{}m}{%
  \begingroup
  \pgfkeys{/TFmacro,#1}%
  \begin{tikzpicture}[baseline=(TFmacroMatrix.center)]
    \matrix[TFmacro/table] (TFmacroMatrix) {%
      #2%
    };
  \end{tikzpicture}%
  \endgroup
}

\NewDocumentCommand{\TFHead}{mmm}{%
  {#1} \& {#2} \& {#3} \\
}

\NewDocumentCommand{\TFRow}{mmm}{%
  {#1} \& {#2} \& {#3} \\
}

\NewDocumentCommand{\TFStripeRow}{mmm}{%
  {#1} \& {#2} \& {#3} \\
}

\NewDocumentCommand{\TFRule}{}{%
  {} \& {} \& {} \\
}

\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colored-letter TF tables 
% ----------------------------------------
%
% Syntax:
%   \vTFtab{4}{{A,D,BC},{A,B,C,D},{B,D,C,A}}
% If no row uses the final position, it can be omitted entirely, using the short key
% np = "no purifier":
% For many rows, use the transposed ("horizontal") version:
%   \vTFtabHor{4}{{A,D,BC},{A,B,C,D},{B,D,C,A}}

\ExplSyntaxOn

\tl_new:N \l__tfmacro_title_tl
\tl_new:N \l__tfmacro_red_word_tl
\tl_new:N \l__tfmacro_green_word_tl
\tl_new:N \l__tfmacro_blue_word_tl
\tl_new:N \l__tfmacro_black_word_tl
\tl_new:N \l__tfmacro_cell_color_tl
\tl_new:N \l__tfmacro_current_letter_tl
\tl_new:N \l__tfmacro_current_row_tl
\tl_new:N \l__tfmacro_last_header_tl
\clist_new:N \l__tfmacro_row_clist
\bool_new:N \l__tfmacro_omit_last_col_bool
\int_new:N \l__tfmacro_col_count_int
\int_new:N \l__tfmacro_row_count_int

\def\TFPatternCellSize{0.34}
\def\TFPatternBoxSize{0.17}
\def\TFPatternHeaderFont{\sffamily\fontsize{6}{12}\selectfont}
\def\TFPatternTitleFont{\rmfamily\fontsize{11}{12}\selectfont}

% Named colors used by the four word positions and by the table frame.
\definecolor{TFPatternRed}{RGB}{255,145,149}
\definecolor{TFPatternGreen}{RGB}{164,246,143}
\definecolor{TFPatternBlue}{RGB}{137,145,239}
\definecolor{TFPatternBlack}{RGB}{0,0,0}
\definecolor{TFPatternGrid}{RGB}{210,210,210}
\definecolor{TFPatternBoxRule}{RGB}{160,160,160}
\definecolor{TFPatternHeaderFill}{RGB}{216,216,216}

\pgfkeys{
  /TFPattern/.is~family,
  /TFPattern,
  title/.code=\tl_set:Nn \l__tfmacro_title_tl {#1},
  last~header/.code=\tl_set:Nn \l__tfmacro_last_header_tl {#1},
  alphabetic~last~header/.code=\tl_clear:N \l__tfmacro_last_header_tl,
  omit~last~column/.code=\bool_set_true:N \l__tfmacro_omit_last_col_bool,
  np/.code=\bool_set_true:N \l__tfmacro_omit_last_col_bool,
  cell~size/.store~in=\TFPatternCellSize,
  box~size/.store~in=\TFPatternBoxSize,
  header~font/.store~in=\TFPatternHeaderFont,
  title~font/.store~in=\TFPatternTitleFont,
  red/.code=\colorlet{TFPatternRed}{#1},
  green/.code=\colorlet{TFPatternGreen}{#1},
  blue/.code=\colorlet{TFPatternBlue}{#1},
  black/.code=\colorlet{TFPatternBlack}{#1},
  grid/.code=\colorlet{TFPatternGrid}{#1},
  box~rule/.code=\colorlet{TFPatternBoxRule}{#1},
  header~fill/.code=\colorlet{TFPatternHeaderFill}{#1}
}

\cs_new:Npn \__tfmacro_letter_label:n #1
  {
    \bool_if:NTF \l__tfmacro_omit_last_col_bool
      { \int_to_Alph:n {#1} }
      {
        \int_compare:nNnTF {#1} = { \l__tfmacro_col_count_int }
          {
            \tl_if_empty:NTF \l__tfmacro_last_header_tl
              { \int_to_Alph:n {#1} }
              { \tl_use:N \l__tfmacro_last_header_tl }
          }
          { \int_to_Alph:n {#1} }
      }
  }

\cs_new_protected:Npn \__tfmacro_set_cell_color:n #1
  {
    \tl_clear:N \l__tfmacro_cell_color_tl
    \tl_if_in:NnT \l__tfmacro_red_word_tl {#1}
      { \tl_set:Nn \l__tfmacro_cell_color_tl {TFPatternRed} }
    \tl_if_empty:NT \l__tfmacro_cell_color_tl
      {
        \tl_if_in:NnT \l__tfmacro_green_word_tl {#1}
          { \tl_set:Nn \l__tfmacro_cell_color_tl {TFPatternGreen} }
      }
    \tl_if_empty:NT \l__tfmacro_cell_color_tl
      {
        \tl_if_in:NnT \l__tfmacro_blue_word_tl {#1}
          { \tl_set:Nn \l__tfmacro_cell_color_tl {TFPatternBlue} }
      }
    \tl_if_empty:NT \l__tfmacro_cell_color_tl
      {
        \tl_if_in:NnT \l__tfmacro_black_word_tl {#1}
          { \tl_set:Nn \l__tfmacro_cell_color_tl {TFPatternBlack} }
      }
  }

\cs_new_protected:Npn \__tfmacro_draw_header_cell:n #1
  {
    \pgfmathsetmacro{\tfmacrox}{(#1 - 1) * \TFPatternCellSize}
    \path[
      draw=TFPatternGrid,
      fill=TFPatternHeaderFill,
      line~width=0.35pt
    ]
      (\tfmacrox,0)
      rectangle
      ++(\TFPatternCellSize,-\TFPatternCellSize);
    \node[
      font=\TFPatternHeaderFont,
      inner~sep=0pt
    ]
      at
      ({\tfmacrox + 0.5 * \TFPatternCellSize},
       {-0.5 * \TFPatternCellSize})
      {\__tfmacro_letter_label:n {#1}};
  }

\cs_new_protected:Npn \__tfmacro_draw_pattern_cell:nn #1#2
  {
    \pgfmathsetmacro{\tfmacrox}{(#2 - 1) * \TFPatternCellSize}
    \pgfmathsetmacro{\tfmacroy}{-#1 * \TFPatternCellSize}
    \path[
      draw=TFPatternGrid,
      fill=white,
      line~width=0.35pt
    ]
      (\tfmacrox,\tfmacroy)
      rectangle
      ++(\TFPatternCellSize,-\TFPatternCellSize);
    \tl_set:Nx \l__tfmacro_current_letter_tl
      { \__tfmacro_letter_label:n {#2} }
    \exp_args:NV \__tfmacro_set_cell_color:n \l__tfmacro_current_letter_tl
    \tl_if_empty:NTF \l__tfmacro_cell_color_tl
      {
        \path[
          draw=TFPatternBoxRule,
          fill=white,
          line~width=0.3pt
        ]
          ({\tfmacrox + 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize},
           {\tfmacroy - 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize})
          rectangle
          ++(\TFPatternBoxSize,\TFPatternBoxSize);
      }
      {
        \path[
          draw=TFPatternBoxRule,
          fill=\l__tfmacro_cell_color_tl,
          line~width=0.3pt
        ]
          ({\tfmacrox + 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize},
           {\tfmacroy - 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize})
          rectangle
          ++(\TFPatternBoxSize,\TFPatternBoxSize);
      }
  }

\cs_new_protected:Npn \__tfmacro_draw_transposed_header_cell:n #1
  {
    \pgfmathsetmacro{\tfmacroy}{-(#1 - 1) * \TFPatternCellSize}
    \path[
      draw=TFPatternGrid,
      fill=TFPatternHeaderFill,
      line~width=0.35pt
    ]
      (0,\tfmacroy)
      rectangle
      ++(\TFPatternCellSize,-\TFPatternCellSize);
    \node[
      font=\TFPatternHeaderFont,
      inner~sep=0pt
    ]
      at
      ({0.5 * \TFPatternCellSize},
       {\tfmacroy - 0.5 * \TFPatternCellSize})
      {\__tfmacro_letter_label:n {#1}};
  }

\cs_new_protected:Npn \__tfmacro_draw_transposed_cell:nnn #1#2#3
  {
    \clist_set:Nn \l__tfmacro_row_clist {#3}
    \tl_set:Nx \l__tfmacro_red_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {1} }
    \tl_set:Nx \l__tfmacro_green_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {2} }
    \tl_set:Nx \l__tfmacro_blue_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {3} }
    \tl_set:Nx \l__tfmacro_black_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {4} }
    \pgfmathsetmacro{\tfmacrox}{#2 * \TFPatternCellSize}
    \pgfmathsetmacro{\tfmacroy}{-(#1 - 1) * \TFPatternCellSize}
    \path[
      draw=TFPatternGrid,
      fill=white,
      line~width=0.35pt
    ]
      (\tfmacrox,\tfmacroy)
      rectangle
      ++(\TFPatternCellSize,-\TFPatternCellSize);
    \tl_set:Nx \l__tfmacro_current_letter_tl
      { \__tfmacro_letter_label:n {#1} }
    \exp_args:NV \__tfmacro_set_cell_color:n \l__tfmacro_current_letter_tl
    \tl_if_empty:NTF \l__tfmacro_cell_color_tl
      {
        \path[
          draw=TFPatternBoxRule,
          fill=white,
          line~width=0.3pt
        ]
          ({\tfmacrox + 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize},
           {\tfmacroy - 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize})
          rectangle
          ++(\TFPatternBoxSize,\TFPatternBoxSize);
      }
      {
        \path[
          draw=TFPatternBoxRule,
          fill=\l__tfmacro_cell_color_tl,
          line~width=0.3pt
        ]
          ({\tfmacrox + 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize},
           {\tfmacroy - 0.5 * \TFPatternCellSize - 0.5 * \TFPatternBoxSize})
          rectangle
          ++(\TFPatternBoxSize,\TFPatternBoxSize);
      }
  }

\cs_new_protected:Npn \__tfmacro_draw_transposed_row:nn #1#2
  {
    \__tfmacro_draw_transposed_header_cell:n {#1}
    \int_step_inline:nn { \l__tfmacro_row_count_int }
      {
        \tl_set:Nx \l__tfmacro_current_row_tl
          { \clist_item:nn {#2} {##1} }
        \exp_args:NnnV \__tfmacro_draw_transposed_cell:nnn
          {#1}
          {##1}
          \l__tfmacro_current_row_tl
      }
  }

\cs_new_protected:Npn \__tfmacro_draw_pattern_row:nn #1#2
  {
    \clist_set:Nn \l__tfmacro_row_clist {#2}
    \tl_set:Nx \l__tfmacro_red_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {1} }
    \tl_set:Nx \l__tfmacro_green_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {2} }
    \tl_set:Nx \l__tfmacro_blue_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {3} }
    \tl_set:Nx \l__tfmacro_black_word_tl
      { \clist_item:Nn \l__tfmacro_row_clist {4} }
    \int_step_inline:nn { \l__tfmacro_col_count_int }
      { \__tfmacro_draw_pattern_cell:nn {#1} {##1} }
  }

\NewDocumentCommand{\vTFtab}{O{}mm}
  {
    \group_begin:
      \tl_clear:N \l__tfmacro_title_tl
      \tl_set:Nn \l__tfmacro_last_header_tl {O}
      \bool_set_false:N \l__tfmacro_omit_last_col_bool
      \pgfkeys{/TFPattern,#1}
      \bool_if:NTF \l__tfmacro_omit_last_col_bool
        { \int_set:Nn \l__tfmacro_col_count_int {#2} }
        { \int_set:Nn \l__tfmacro_col_count_int { #2 + 1 } }
      \begin{tikzpicture}[x=1cm,y=1cm,baseline=(current~bounding~box.center)]
        \pgfmathsetmacro{\tfmacrotablewidth}
          {\int_use:N \l__tfmacro_col_count_int * \TFPatternCellSize}
        \tl_if_empty:NF \l__tfmacro_title_tl
          {
            \node[
              font=\TFPatternTitleFont,
              inner~sep=0pt
            ]
              at ({0.5 * \tfmacrotablewidth},{0.34})
              {\tl_use:N \l__tfmacro_title_tl};
          }
        \int_step_inline:nn { \l__tfmacro_col_count_int }
          { \__tfmacro_draw_header_cell:n {##1} }
        \int_zero:N \l__tfmacro_row_count_int
        \clist_map_inline:nn {#3}
          {
            \int_incr:N \l__tfmacro_row_count_int
            \__tfmacro_draw_pattern_row:nn
              { \l__tfmacro_row_count_int }
              {##1}
          }
      \end{tikzpicture}
    \group_end:
  }

\NewDocumentCommand{\vTFtabHor}{O{}mm}
  {
    \group_begin:
      \tl_clear:N \l__tfmacro_title_tl
      \tl_set:Nn \l__tfmacro_last_header_tl {O}
      \bool_set_false:N \l__tfmacro_omit_last_col_bool
      \pgfkeys{/TFPattern,#1}
      \bool_if:NTF \l__tfmacro_omit_last_col_bool
        { \int_set:Nn \l__tfmacro_col_count_int {#2} }
        { \int_set:Nn \l__tfmacro_col_count_int { #2 + 1 } }
      \int_set:Nn \l__tfmacro_row_count_int { \clist_count:n {#3} }
      \begin{tikzpicture}[x=1cm,y=1cm,baseline=(current~bounding~box.center)]
        \pgfmathsetmacro{\tfmacrotablewidth}
          {(\int_use:N \l__tfmacro_row_count_int + 1) * \TFPatternCellSize}
        \tl_if_empty:NF \l__tfmacro_title_tl
          {
            \node[
              font=\TFPatternTitleFont,
              inner~sep=0pt
            ]
              at ({0.5 * \tfmacrotablewidth},{0.34})
              {\tl_use:N \l__tfmacro_title_tl};
          }
        \int_step_inline:nn { \l__tfmacro_col_count_int }
          { \__tfmacro_draw_transposed_row:nn {##1} {#3} }
      \end{tikzpicture}
    \group_end:
  }

\NewDocumentCommand{\TFPatternTable}{O{}mm}{\vTFtab[#1]{#2}{#3}}
\NewDocumentCommand{\TFPatternTableTranspose}{O{}mm}{\vTFtabHor[#1]{#2}{#3}}

\ExplSyntaxOff

